Low-Complexity Soft-Output MIMO Detectors Based on Optimal Channel Puncturing

Channel puncturing transforms a multiple-input multiple-output (MIMO) channel into a sparse lower-triangular form using the so-called WL decomposition scheme in order to reduce tree-based detection complexity. We propose computationally efficient soft-output detectors based on two forms of channel puncturing: augmented and two-sided. The augmented WL detector (AWLD) employs a punctured channel derived by triangularizing the true channel in augmented form, followed by leftsided Gaussian elimination. The two-sided WL detector (dubbed WLZ) employs right-sided reduction and left-sided elimination to puncture the channel. We prove that augmented channel puncturing is optimal in maximizing the lower-bound on the achievable information rate (AIR) based on a new mismatched detection model. We show that the AWLD decomposes into an MMSE prefilter and channel gain compensation stages, followed by a regular WL detector (WLD) that computes least-squares softdecision estimates. Similarly, WLZ decomposes into a pre-processing reduction step followed by WLD. AWLD attains the same performance as the existing AIR-based partial marginalization (PM) detector, but with less computational complexity. We empirically show that WLZ attains the best complexityperformance tradeoff among tree-based detectors.

==> awld_block_diagram_2col.tex <==
\tikzstyle{int}=[draw, fill=blue!20, minimum size=2em]
\tikzstyle{init} = [pin edge={to-,thin,black}]

\begin{tikzpicture}[node distance=2.75cm, auto, >=latex', pin distance = 3mm]
    \node [int, pin={[init]above:{\small$\H,\beta$}}, label=below:{\scriptsize MMSE
    filter}] (a) {{\small$\Wmmse$\normalsize}};

    \node (b) [left of=a,node distance=0.9cm, coordinate] {};

    \node [int, pin={[init]above:{\small$\Ha$}}] (c) [right of=a,  label=below:{\scriptsize Gain compensation}, node distance=1.8cm] {{\small$\Lap$\normalsize}};

    \node [int, pin={[init]above:{\small$\Lap$}}, label=below:{\scriptsize WLD detector}] (d) [right of=c, node distance=3.4cm] {{\small$\arg\max\tfrac{1}{\Es}\fnormmsq{\x}\!-\! \fnormmsq{\yap\!-\!\Lap\x}$\normalsize}};

    \node [coordinate] (end) [right of=d, node distance=2.7cm]{};

    \path[->] (b) edge node {{\small$\y$}} (a);
    \path[->] (a) edge node {{\small$\Wmmse\y$\normalsize}} (c);
    \draw[->] (c) edge node {{\small$\yap$\normalsize}} (d);
    \draw[->] (d) edge node {{\small$\hat{\x}$}} (end);

\end{tikzpicture} 

==> network.tex <==
\begin{tikzpicture}
\matrix (network)
[matrix of nodes,%
nodes in empty cells,
nodes={outer sep=0pt,circle,minimum size=4pt,draw},
column sep={1cm,between origins},
row sep={1cm,between origins}]
{
& & & \\
& & & \\
|[draw=none]| & |[xshift=1mm]| & |[xshift=-1mm]| \\
};
\foreach \a in {1,...,4}{
\draw (network-3-2) -- (network-2-\a);
\draw (network-3-3) -- (network-2-\a);
\draw [-stealth] ([yshift=5mm]network-1-\a.north) -- (network-1-\a);
\foreach \b in {1,...,4}
\draw (network-1-\a) -- (network-2-\b);
}
\draw [stealth-] ([yshift=-5mm]network-3-2.south) -- (network-3-2);
\draw [stealth-] ([yshift=-5mm]network-3-3.south) -- (network-3-3);
\end{tikzpicture}


==> wdl_H.tex <==
% ------------------------ Matlab: wdl_H.m function --------------------------
\begin{algorithm}
\small
\caption{WDL decomposition algorithm}\label{algo:wdl}
\begin{algorithmic}[0]
\FunctionRV{WL}{\H,\y,\nu}{\Lptilde, \Dp, \yptilde, \Wptilde}\Comment{$\H\!:\Nr\!\times\!\Nt$}
\State $\Ltilde\gets \mbf{0}_{\Nt\times{(\Nt+1)}}^{}$
\State $\Qtilde\gets[\y ~ \H]$ \Comment{\textit{Augmented matrix}}
\State $\Dp \gets \mbf{0}_{\Nt\times\Nt}^{}$
% --------------- QDL decomposition ----------------------------
\For{$i\!=\!\Nt\!+\!1\!:\!-1\!:\!2$}\Comment{\textit{QDL decomposition}: $\H\!=\!\Qtilde\Dp\Ltilde$}
    \State $\Dp(i\!-\!1,i\!-\!1) \gets \Qtilde(:,i)^{\dag}\Qtilde(:,i)$
    \For{$j\!=\!i\!-\!1\!:\!-1\!:\!1$}
        \State $\Ltilde(i\!-\!1,j) \!\gets\! \Qtilde(:,i)^{\dag}\Qtilde(:,j) / \Dp(i\!-\!1,i\!-\!1)$
        \State $\Qtilde(:,j) \!\gets\! \Qtilde(:,j) \!-\! \Ltilde(i\!-\!1,j)\Qtilde(:,i)$
    \EndFor\label{WLendforb}
    \State $\Qtilde(:,i) \!\gets\! \Qtilde(:,i) / \Dp(i\!-\!1,i\!-\!1)$
\EndFor\label{WLendfora}\Comment{\textit{now} $\yptilde \!=\! \Qtildeh\y \!=\! \subpsc{\mbf{D}}{\mathrm{p}}{\,-1/2}\Qh\y$}
% -------------- Gaussian elimination --------------------------
\For{$i\!=\!\nu\!+\!2\!:\!\Nt$}\Comment{\textit{Gaussian elimination}}
    \For{$j\!=\!\nu\!+\!1\!:\!i\!-\!1$} \Comment{\textit{col index to puncture}}
        \State{$\alpha \!\gets\! \Ltilde(i,j\!+\!1)$}
        \State $\Qtilde(:,i\!+\!1) \!\gets\! \Qtilde(:,i\!+1) \!-\! \alpha^{\dag}\Qtilde(:,j\!+\!1)$
        \State $\Ltilde(i,1\!:\!j\!+\!1) \!\gets\! \Ltilde(i,1\!:\!j\!+\!1) \!-\! \alpha \Ltilde(j,1\!:\!j\!+\!1)$
    \EndFor\label{WLendforc}
    \State $\Dp(i,i) \!\gets\! 1/(\Qtilde(:,i\!+\!1)^{\dag} \Qtilde(:,i\!+\!1) )$
\EndFor\label{WLendford}
\State $\yptilde \!\gets\! \Ltilde(:,1)$
\State $\Lptilde \!\gets\! \Ltilde(:,2\!:\!\Nt\!+\!1)$
\State $\Wptilde \!\gets\! \Qtilde(:,2\!:\!\Nt\!+\!1)^{\dag}$\Comment{\textit{take conjugate transpose}}
\EndFunctionRV
\end{algorithmic}
\end{algorithm}





==> wld.tex <==
%% -------------------------------------------------------------------------
%% -- WL decomposition
%% -- H: m x n; m >= n
%% -- y: m x 1
%% -- Generate W matrix s.t. Wp'*H = Lp, Wp'*y = yt and diag(Wp'*Wp) = I
%% -- Lp: punctured lower-triangular matrix with pos real diagonal entries
%% -- 2017 (c) Mohammad Mansour, mmansour@ieee.org
%% -------------------------------------------------------------------------
%function [Lp, yt, Wp] = wld(H, y, v)
%if nargin==2, v=1; end
%[~,n] = size(H);
%Lp = zeros(n,n+1);
%Q = [y H];
%
%for i=n+1:-1:2
%    Lp(i-1,i) = sqrt(Q(:,i)'*Q(:,i));
%    Q(:,i) = Q(:,i)/Lp(i-1,i);
%    for j=i-1:-1:1
%        Lp(i-1,j) = Q(:,i)'*Q(:,j);
%        Q(:,j) = Q(:,j) - Lp(i-1,j)*Q(:,i);
%    end
%end
%
%for i=v+1:n
%    for j=v+1:i-1
%        alpha = Lp(i,j+1)/Lp(j,j+1);
%        Q(:,i+1) = Q(:,i+1) - alpha'*Q(:,j+1);
%        Lp(i,1:j+1) = Lp(i,1:j+1) - alpha*Lp(j,1:j+1);
%    end
%    Lp(i,1:i+1) = Lp(i,1:i+1) / norm(Q(:,i+1));
%    Q(:,i+1) = Q(:,i+1) / norm(Q(:,i+1));
%end
%
%yt = Lp(:,1);
%Lp = Lp(:,2:end);
%Wp = Q(:,2:end);

\begin{algorithm}
\small
\caption{WL decomposition algorithm}\label{algo:wl}
\begin{algorithmic}[0]
\FunctionRV{WL}{\H,\y,\nu}{\Lp, \yt, \Wp}\Comment{$\H:\Nr\!\times\!\Nt$}
\State $\Lp\gets \mbf{0}_{\Nt\times{(\Nt+1)}}^{}$
\State $\Q\gets[\y ~ \H]$
\For{$i\!=\!\Nt\!+\!1\!:\!-1\!:\!2$}\Comment{QL decomposition}
    \State $\Lp\!(i\!-\!1,i) \gets \sqrt{\Q(:,i)^{\dag}\Q(:,i)}$
    \State $\Q(:,i) \!=\! \Q(:,i)/\Lp(i\!-\!1,i)$
    \For{$i\!=\!\Nt\!+\!1\!:\!-1\!:\!2$}
        \State $\Lp(i\!-\!1,j) \!\gets\! \Q(:,i)^{\dag}\Q(:,j)$
        \State $\Q(:,j) \!\gets\! \Q(:,j) \!-\! \Lp(i\!-\!1,j)\Q(:,i)$
    \EndFor\label{WLendforb}
\EndFor\label{WLendfora}
\For{$i\!=\!\nu\!+\!1\!:\!\Nt$}\Comment{Gaussian elimination}
    \For{$j\!=\!\nu\!+\!1\!:\!i\!-\!1$}
        \State{$\alpha \!\gets\! \Lp(i,j\!+\!1)/\Lp(j,j\!+\!1)$}
        \State $\Q(:,i\!+\!1) \!\gets\! \Q(:,i\!+1) \!-\! \alpha^*\Q(:,j\!+\!1)$
        \State $\Lp(i,1\!:\!j\!+\!1) \!\gets\! \Lp(i,1\!:\!j\!+\!1) \!-\! \alpha \Lp(j,1\!:\!j\!+\!1)$
    \EndFor\label{WLendforc}
    \State $\Lp(i,1\!:\!i\!+\!1) \!\gets\! \Lp(i,1\!:\!i\!+\!1) / \norm{\Q(:,i\!+\!1)}$
    \State $\Q(:,i\!+\!1) \!\gets\! \Q(:,i\!+\!1) / \norm{\Q(:,i\!+\!1)}$
\EndFor\label{WLendford}
\State $\yt \!\gets\! \Lp(:,1)$
\State $\Lp \!\gets\! \Lp(:,2\!:\!\Nt\!+\!1)$
\State $\Wp \!\gets\! \Q(:,2\!:\!\Nt\!+\!1)$
\EndFunctionRV
\end{algorithmic}
\end{algorithm} 




